Video Prediction Policy: A Generalist Robot Policy with Predictive Visual Representations

Visual representations play a crucial role in developing generalist robotic policies. Previous vision encoders, typically pre-trained with single-image reconstruction or two-image contrastive learning, tend to capture static information, often neglecting the dynamic aspects vital for embodied tasks. Recently, video diffusion models (VDMs) demonstrate the ability to predict future frames and showcase a strong understanding of physical world. We hypothesize that VDMs inherently produce visual representations that encompass both current static information and predicted future dynamics, thereby providing valuable guidance for robot action learning. Based on this hypothesis, we propose the Video Prediction Policy (VPP), which learns implicit inverse dynamics model conditioned on predicted future representations inside VDMs. To predict more precise future, we fine-tune pre-trained video foundation model on robot datasets along with internet human manipulation data. In experiments, VPP achieves a 18.6\% relative improvement on the Calvin ABC-D generalization benchmark compared to the previous state-of-the-art, and demonstrates a 31.6\% increase in success rates for complex real-world dexterous manipulation tasks. Project page at https://video-prediction-policy.github.io

==> sec/X_figure.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/1-1.png}
    \caption{moving bottle away from bottle}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/1-2.png}
    \caption{moving silicone towards the camera}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/1-3.png}
    \caption{moving toy closer to plastic glass}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/1-4.png}
    \caption{pouring liquid into a cup}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/1-5.png}
    \caption{pouring milk into glass}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/1-6.png}
    \caption{turning the camera right while filming jeep}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/1-7.png}
    \caption{pretending to pick a tennis ball up}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/1-8.png}
    \caption{pulling toy car from left to right}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/1-9.png}
    \caption{putting something similar}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/1-10.png}
    \caption{tearing paper into two pieces}
    \end{subfigure}
    
    \caption{\textbf{Visualization of video prediction results on Internet human manipulation validation datasets with 30 steps de-noising}. The green frames indicate the ground truth while the red frames indicate the predicted futures. Zoom in for better comparisons.}
    \label{svd_human}
\end{figure}


\begin{figure}
    \centering
    % \begin{subfigure}[h]{0.49\textwidth}
    % \includegraphics[width=\linewidth]{fig_sthv2/robot_close microwave_6_.png}
    % \caption{close microwave}
    % \end{subfigure}
    % \begin{subfigure}[h]{0.49\textwidth}
    % \includegraphics[width=\linewidth]{fig_sthv2/robot_Move the yellow towel to the right of the blue ladle_5_.png}
    % \caption{Move the yellow towel to the right of the blue ladle}
    % \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-1.png}
    \caption{open bottom drawer}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-2.png}
    \caption{place apple into bottom drawer}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-3.png}
    \caption{place eraser in purple bowl}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-4.png}
    \caption{place the white sponge in the ceramic cup}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-5.png}
    \caption{put bowl on plate cardboard fence}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-6.png}
    \caption{put eggplant into pot or pan}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-7.png}
    \caption{Place the grasped object into the drawer}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-8.png}
    \caption{close the drawer}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-9.png}
    \caption{Put the grey circle on the red pole}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-10.png}
    \caption{open the drawer}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-11.png}
    \caption{pick carrot}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-12.png}
    \caption{pick the blue block}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-13.png}
    \caption{Put the green block above the red block}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-14.png}
    \caption{Place the purple onion onto the basket}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-15.png}
    \caption{pick the yellow ball to the empty hole of the board}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{fig_sthv2/2-16.png}
    \caption{Receive the orange from hand and place it into the basket}
    \end{subfigure}
    \caption{\textbf{Visualization of video prediction results on robotic datasets with 30 steps de-noising}. The green frames indicate the ground truth while the red frames indicate the predicted futures. (a)-(j) are sourced from internet robotic while (k)-(p) are from self-collected datasets. Zoom in for better comparisons.}
    \label{svd_robot}
\end{figure}


\begin{figure}
    \centering
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{step1/frame_test_calvin_1_10.png}
    \caption{place the grasped object in the drawer.}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{step1/frame_test_calvin_1_12.png}
    \caption{close the drawer.}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{step1/3-1.png}
    \caption{pick the mango and place in blue plate}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=\linewidth]{step1/3-2.png}
    \caption{stack the green block on red block}
    \end{subfigure}

    \caption{\textbf{Visualization of Predictive representations}. Green frames represent the ground truth, red frames correspond to the predicted future states, and blue frames illustrate the visualized predictive representations. Zoom in for better comparisons.}
    \label{svd_step1}
\end{figure}
